Grid Obstacle Representation of Graphs

The grid obstacle representation, or alternately, $\ell_1$-obstacle representation of a graph $G=(V,E)$ is an injective function $f:V \rightarrow \mathbb{Z}^2$ and a set of point obstacles $\mathcal{O}$ on the grid points of $\mathbb{Z}^2$ (where no vertex of $V$ has been mapped) such that $uv$ is an edge in $G$ if and only if there exists a Manhattan path between $f(u)$ and $f(v)$ in $\mathbb{Z}^2$ avoiding the obstacles of $\mathcal{O}$ and points in $f(V)$. This work shows that planar graphs admit such a representation while there exist some non-planar graphs that do not admit such a representation. Moreover, we show that every graph admits a grid obstacle representation in $\mathbb{Z}^3$. We also show NP-hardness result for the point set embeddability of an $\ell_1$-obstacle representation.

==> obstacle-3dimension.tex <==


\section{Grid obstacle representation in $3$-dimension}
\label{app:embedding3D}

In this section, we show the existence of obstacle representation in three dimension. The proof of the existential result is based on the following theorem by Pach \emph{et al.}~\cite{PachTT97}.

\begin{theo}[\cite{PachTT97}] \label{theo:Pach3dim}
For every fixed $r\geq 2$, any $r$-colorable graph with $n$ vertices has a straight line embedding in $\mathbb{Z}^3$ in $O(r)\times O(n)\times O(rn)$ grid.
\end{theo}

First, we construct a straight line embedding of an $r$-colorable graph in a refined grid such that the distance between a vertex $v$ and a straight line edge $e$ not containing $v$ is \emph{sufficiently large}. To do that, we give a bound on the minimum distance of a grid point from a straight line edge in the embedding that is obtained from Theorem \ref{theo:Pach3dim}. Clearly this distance is smaller than or equal to the distance of a vertex from a straight line edge. Using similar argument as in Section \ref{sec:embedding}, we get that the minimum distance of a grid point from a straight line edge is $O(1/rn)$, where $r$ is the chromatic number of the graph. Now we blow the grid uniformly by a factor of $\mathcal{C}.rn$ such that the distance between a vertex $v$ and a straight line edge $e$ not containing $v$ becomes greater than a constant $\mathcal{C}$. Hence, we have the following lemma.

\begin{lem}\label{lem:stlineon3dim}
Every $r$-colorable graph admits a straight line embedding in $O(r^2n)\times O(rn^2)\times O(r^2n^2)$ grid such that two vertices are at least a distance $\mathcal{C}$ apart and a vertex and an edge are also at least a distance $\mathcal{C}$ apart, where $\mathcal{C}$ is a constant.
\end{lem}

The idea of the proof is similar to the proof presented in Section \ref{sec:embedding}. The idea is as follows:

\begin{description}
\item[1.] Obtain a straight line embedding of a $r$-colorable graph as in Lemma~\ref{lem:stlineon3dim}.

\item[2.] Consider an $\epsilon$-cube $C^{\epsilon}(v)$, a cube of length $\epsilon$, around each vertex $v$ such that
\begin{itemize}
  \item for two distinct vertices $u$ and $v$, $C^{\epsilon}(v) \cap C^{\epsilon}(u) = \emptyset$,
  \item distance between two $\epsilon$-cubes $C^{\epsilon}(u)$ and $C^{\epsilon}(v)$ is large (say $q_1$), and
  \item distance between an $\epsilon$-cube $C^{\epsilon}(v)$ and a straight line edge $e$ not containing $v$ is also adequate (at least $q_2$).
\end{itemize}

\item[3.] Consider a $\delta$-tube $T^{\delta}(e)$ (where $T^{\delta}(e)$ is the Minkowski sum of the embedded edge $e$ and a disk of radius $\delta$) around each straight line edge $e$ such that
\begin{itemize}
  \item for each pair of disjoint straight line edges $e_1$ and $e_2$, $T^{\delta}(e_1) \cap T^{\delta}(e_2)=\emptyset$,
  \item for each pair of distinct straight line edges $e_1$ and $e_2$ sharing a common vertex $v$, $(T^{\delta}(e_1) \cap T^{\delta}(e_2)) \subset C^{\epsilon}(v)$, and
  \item for a vertex $v$ and a straight line edge $e$ not containing $v$, $C^{\epsilon}(v)\cap T^{\delta}(e)=\emptyset$.
\end{itemize}

\item[4.] Refine the grid in such a way that we can digitize the straight line edge $e$ into a Manhattan path that lies inside $T^{\delta}(e)$.
\end{description}


Now, let us consider $\epsilon$ to be $\ll \mathcal{C}$, where $\mathcal{C}$ is the constant given in Lemma \ref{lem:stlineon3dim}. The value of $\epsilon$ is chosen in such a way that both $q_1=(\mathcal{C} - \epsilon)$ and $q_2=(\mathcal{C}- \sqrt{2}\epsilon)$ are adequately large constant. Next, we fix the $\delta$ to be a constant such that $\delta < \frac{1}{10} \min\limits_{v\in V}\{\delta(v)\}$, where $\delta(v)$ is the minimum Euclidean distance between consecutive intersection points of $C^{\epsilon}(v)$ and straight line edges $e$ containing $v$. The choice of $\delta$ guarantees the following observations about $C^{\epsilon}(v)$ and $T^{\delta}(e)$.

\begin{obs}\label{obs:tubeproperty_on_3}
For the particular choices of $\epsilon$ and $\delta$, the following properties of $T^{\delta}(e)$ and $C^{\epsilon}(v)$ are true:
\begin{itemize}
  \item[1.] For each pair of disjoint straight line edges $e_1$ and $e_2$, $T^{\delta}(e_1) \cap T^{\delta}(e_2)=\emptyset$.
  \item[2.] For each pair of distinct straight line edges $e_1$ and $e_2$ sharing a common vertex $v$, $(T^{\delta}(e_1) \cap T^{\delta}(e_2)) \subset C^{\epsilon}(v)$, i.e., there is no intersection between $\delta$-tubes outside the $\epsilon$-cubes.
  \item[3.] For a vertex $v$ and a straight line edge $e$ not containing $v$, $C^{\epsilon}(v)\cap T^{\delta}(e)=\emptyset$.
\end{itemize}
\end{obs}

Now refine the grid sufficiently until the length of each grid edge becomes $\delta /100$. This is done to ensure that there are enough grid points within $T^{\delta}(e)$ to convert the edge $e$ into a Manhattan path inside $T^{\delta}(e)$. The digitization of a straight line edge $e$ connecting $u$ and $v$ into a Manhattan path $M(e)$ between $u$ and $v$ is done in the similar way as in Lemma~\ref{lem:stline_to_Manhat} in Section \ref{sec:embedding}. After this step, we get an embedding of a $r$ colorable graph in $O(r^2n/\delta)\times O(rn^2/\delta)\times O(r^2n^2/\delta)$ grid where each edge $e$ is represented by a Manhattan path $M(e)$. Now, for fixing the value of $\delta$, we proceed is a similar way as in Lemma \ref{lem:deltavalue} and we get that $\delta=\frac{\mathcal{C'}}{r^2n^2}$, where $\mathcal{C'}$ is a constant and $r$ is the chromatic number of the graph. Hence, we have obtained an embedding of a $r$ chromatic graph on a refined grid of size $O(r^4n^3)\times O(r^3n^4)\times O(r^4n^4)$, where each edge $e$ is represented by a Manhattan path $M(e)$. Also the digitization of the straight line edge is done in such a way that it avoids the edges of the cube $C^{\epsilon}(v)$.

\begin{figure}[!h]

\centering
\includegraphics[scale=0.6]{3d.pdf} \\
\caption{Modification of a Manhattan path inside $C^{\epsilon}(v)$.\\}
\label{fig:3d}
\centering

\end{figure}
Next, we modify the Manhattan paths inside $C^{\epsilon}(v)$ in the way as shown in Figure~\ref{fig:3d}. For each square face $F$ of $C^{\epsilon}(v)$, let $c(F)$ be the point of intersection of the diagonals of $F$. Each Manhattan path $M(e)$ enters the cube $C^{\epsilon}(v)$ through a point, say $x$, on some square face $F$ of $C^{\epsilon}(v)$. Now, alter the portion of the Manhattan path $M(e)$ inside $C^{\epsilon}(v)$ follows: (i) take any Manhattan path from $x$ to $c(F)$ and then (ii) take the straight line path from $c(F)$ to $v$. We do this modification for every Manhattan paths inside $C^{\epsilon}(v)$. Now we place obstacles on the edges of $C^{\epsilon}(v)$ and everywhere inside the cube $C^{\epsilon}(v)$ except square faces and the axis parallel straight lines containing $v$. We do this modification for every cube $C^{\epsilon}(v)$. The Manhattan path $M(e)$ between $u$ and $v$ is now modified to another path containing the altered path inside $C^{\epsilon}(u)$, followed by the portion of $M(e)$ outside $C^{\epsilon}(u)$ and $C^{\epsilon}(v)$, and finally the altered path inside $C^{\epsilon}(v)$. Next we place obstacles on each empty grid point throughout the grid. Note that the modified paths are also Manhattan paths. Hence, we have the following theorem.

\begin{theo}\label{theo:3d}
Every $r$ colorable graph admits a $(\mathbb{Z}^{3}, \ell_1)$ obstacle representation in $O(r^4n^3)\times O(r^3n^4)\times O(r^4n^4)$ grid.
\end{theo}



==> obstacle-ProofLemma6.tex <==
\section{Proof of Lemma \ref{lem:deltavalue}}
\label{sec:appendlemma}

\begin{proof}
Let $\delta (v)$ be as earlier and let it be achieved by two straight line edges $vu$ and $vw$. Let $A$ and $B$ be the two points where the boundary of $B^{\epsilon}(v)$ intersects with $vu$ and $vw$ respectively. Hence, $\delta(v)=\overline{AB}$.

\begin{figure}[!h]
\vspace{-20pt}
\begin{center}
\includegraphics[width=6cm]{deltavalue.pdf}
\caption{Fixing the value of $\delta$ in the $O(n^2) \times O(n^2)$ grid\\.}
\label{fig:deltavalue}
\end{center}
\vspace{-25pt}
\end{figure}


\noindent\textbf{Case 1:}
Assume that $A$ and $B$ are on the same side of $B^{\epsilon}(v)$ and both $vu$ and $vw$ have positive slope, as shown in the Figure \ref{fig:deltavalue}. Let $uP$ be the perpendicular on $vw$ and $uQ$ be parallel to $AB$. Note that, $vA > \epsilon/2$. By Lemma \ref{lem:stlineOn2}, $uP > \mathcal{C}$. So, clearly $uQ > \mathcal{C}$. Since, the grid is of size $O(n^2)\times O(n^2)$, we have $vu < \mathcal{C}_1\cdot n^2$. Now, as $\triangle vAB$ and $\triangle vuQ$ are similar, we have,
$$\frac{AB}{vA}= \frac{uQ}{vu} \Rightarrow AB > \frac{ \epsilon \mathcal{C}}{2\mathcal{C}_1}\cdot 1/n^2$$


\begin{figure}[!h]
\vspace{-20pt}
\begin{center}
\includegraphics[width=5cm]{deltavalue2.pdf}
\caption{Fixing the value of $\delta$ in the $O(n^2) \times O(n^2)$ grid.}
\label{fig:deltavalue2}
\end{center}
\vspace{-20pt}
\end{figure}


\noindent\textbf{Case 2:} Assume that $A$ and $B$ are on the same side of $B^{\epsilon}(v)$ and $vu$ is of positive slope and $vw$ is of negative slope, as shown in the Figure \ref{fig:deltavalue2}. This case can be handled in a similar way.

\noindent\textbf{Case 3:} Assume that $A$ and $B$ are on two consecutive sides of $B^{\epsilon}(v)$, as shown in the Figure \ref{fig:deltavalue3}. Let $AA'$ and $uQ$ be two perpendiculars on $vw$. In this case, $AB > AA'$. Using the similarity of $\triangle vAA'$ and $\triangle vuQ$, we have $AA' > \mathcal{C_2} \cdot 1/n^2$. Since $AB > AA'$, we have $\delta(v)> \mathcal{C_2} \cdot 1/n^2$.
\begin{figure}[!h]
\vspace{-20pt}
\begin{center}
\includegraphics[width=5cm]{deltavalue3.pdf}
\caption{Fixing the value of $\delta$ in the $O(n^2) \times O(n^2)$ grid.}
\label{fig:deltavalue3}
\end{center}
\vspace{-20pt}
\end{figure}

Hence, by choosing an appropriate constant, we have $\delta = \mathcal{C'} \cdot 1/n^2 $ for all cases.
\end{proof}


==> obstacle-example.tex <==


\section{Examples of grid obstacle representations}
\label{app:examplesgridrepresentation}
Here we present $\ell_1$-obstacle representation of a few graph classes. In some cases, we show that the $\ell_1$-obstacle representation uses minimum number of obstacles and in rest of the cases, the $\ell_1$-obstacle representation gives an upper bound on $\ell_1$-obstacle number. In all the following figures, the Manhattan edges of the $\ell_1$-obstacle representation are not shown if it is obvious.

\subsection{Path $P_n$, cycle $C_n$ and matching $M$}
For a path $P_n$ on $n$ vertices, the $\ell_1$-$obs(P_n)=0$. If we place the
vertices on consecutive grid points of a horizontal or a vertical line, then
each intermediate vertex will act as an obstacle and prevent the edges going
from its previous vertex to all the successive vertices. The $\ell_1$-obstacle
representation of $P_n$ is illustrated in Figure~\ref{fig:path}(a). For a cycle
$C_n$ on $n\geq 7$ vertices, $\ell_1$-$obs(C_n) \leq \ceil{n/2}-3$.
The $\ell_1$-obstacle representation is shown in Figure \ref{fig:path}(b).
For a matching $M_k$ of size $k$, $\ell_1$-$obs(M_k) \leq 2(k-1)$. The
$\ell_1$-obstacle representation is shown in Figure \ref{fig:path}(c).

\begin{figure}[!h]
\centering

\begin{minipage}{0.5\textwidth}
\centering
\includegraphics[width=6cm]{path.pdf} \\
{(a) $\ell_1$-obstacle representation of $P_{10}$.\\}
\end{minipage}%
\begin{minipage}{0.5\textwidth}
\centering
\includegraphics[width=6cm]{cycle.pdf} \\
{(b) $\ell_1$-obstacle representation of $C_{26}$. \\}
\end{minipage}

\vspace*{0.3in}

\begin{minipage}{1.0\textwidth}
\centering
\includegraphics[width=9cm]{matching.pdf} \\
{(c) $\ell_1$-obstacle representation of $M_{6}$.\\}
\end{minipage}


\caption{$\ell_1$-obstacle representations of $P_{10}$, $C_{26}$ and $M_{6}$.
Dots represent vertices and the boxes represent the obstacles. We follow this
convention throughout.}
\label{fig:path}
\end{figure}

\remove{
\begin{figure}[!h]
\begin{center}
\includegraphics[width=8cm]{path.pdf}
\end{center}
\caption{$\ell_1$-obstacle representation of $P_{10}$}
\label{fig:path}
\end{figure}
}



\remove{
\begin{figure}[!h]
\begin{center}
\includegraphics[width=8cm]{cycle.pdf}
\caption{$\ell_1$-obstacle representation of $C_{26}$. Dots represent vertices and the boxes represent the obstacles. We follow this convention throughout.}
\label{fig:cycle}
\end{center}
\end{figure}
}



\remove{
\begin{figure}[!h]
\begin{center}
\includegraphics[width=8cm]{matching.pdf}
\caption{$\ell_1$-obstacle representation of $M_{6}$}
\label{fig:matching}
\end{center}
\end{figure}
}

\subsection{Complete graph $K_n$, Complete bipartite graph $K_{n,m}$ and $K_n \setminus M$}
\begin{figure}[!h]
\centering

\begin{minipage}{0.5\textwidth}
\centering
\includegraphics[width=4cm]{complete.pdf} \\
{(a) $\ell_1$-obstacle representation of $K_{12}$.\\}
\end{minipage}%
\begin{minipage}{0.5\textwidth}
\centering
\includegraphics[width=5cm]{bipartite.pdf} \\
{(b) $\ell_1$-obstacle representation of $K_{5,7}$. \\}
\end{minipage}

\caption{$\ell_1$-obstacle representations of $K_{12}$ and $K_{5,7}$.}
\label{fig:complete}
\end{figure}

\remove{
\begin{figure}[!h]
\begin{center}
\includegraphics[width=4cm]{complete.pdf}
\caption{$\ell_1$-obstacle representation of $K_{12}$}
\label{fig:complete}
\end{center}
\end{figure}
}
For a complete graph $K_n$ with $n$ vertices, $\ell_1$-$obs(K_n)=0$, since no
edge has to be blocked. Figure \ref{fig:complete}(a) shows $\ell_1$-obstacle
representation for $K_n$ on $O(n)\times O(n)$ grid, where the vertices are
placed along the edges of a square (convex position is good enough). Actually,
the minimum grid size required for $\ell_1$-obstacle representation is
$\Omega(n)\times \Omega(n)$. Because in this case, no three vertices can be in
same horizontal or vertical line and hence, we need at least $n/2$ horizontal
and $n/2$ vertical lines.



For a complete bipartite graph $K_{n,m}$ with $n$ vertices in one part and $m$
vertices in the other part ($n\leq m$), $\ell_1$-$obs(K_{n,m}) \leq n+m-3$. This
can be done by placing $m$ vertices and $m-1$ obstacles alternately along a
horizontal line and the $n$ vertices of the other part are divided into two
parts and placed along the horizontal lines above and below the horizontal line
of the $m$ vertices. This representation is shown in
Figure~\ref{fig:complete}(b).

\remove{
\begin{figure}[!h]
\begin{center}
\includegraphics[width=7cm]{bipartite.pdf}
\caption{$\ell_1$-obstacle representation of $K_{5,7}$}
\label{fig:bipartite}
\end{center}
\end{figure}
}


\begin{figure}[h]
\vspace{20pt}
\begin{center}
\includegraphics[width=4cm]{comlt_match.pdf}
\vspace{10pt}
\caption{$\ell_1$-obstacle representation of $K_{12} \setminus M_3$}
\label{fig:cmplt_match}
\end{center}
\end{figure}


Given a matching $M_k$ of size $k\geq 2$, we can represent $K_n \setminus M_k$ with at most $(k-1)$ obstacles. In this case, we place the vertices in a convex position as it is in the case of complete graph keeping in mind that the vertices of a matching edge should be in the same horizontal or vertical line. This representation is shown in Figure \ref{fig:cmplt_match}.



\subsection{$\overline{K}_n$ and $\overline{K}_{n,m}$}

It is an interesting open problem to decide whether the $\ell_2$-obstacle number of $\overline{K}_{n}$ is $O(n)$ or not, where the obstacles are point obstacle~\cite{PachS11}. But, in case of $\ell_1$-obstacle number, we can achieve this bound by simply placing obstacles at four grid points around every vertex. In fact, in Figure \ref{fig:complement_complete}, we give an $\ell_1$-obstacle representation with $n-1$ obstacles and we can show that $\ell_1$-$obs(\overline{K}_n)= n-1$. The proof is based on the fact that any graph $G$ with $n$ vertices has at least $n-1$ Manhattan edges when $\ell_1$-$obs(G)= 0$.

\begin{figure}[h]
\vspace{10pt}
\begin{center}
\includegraphics[width=8cm]{complement_complete.pdf}
\caption{$\ell_1$-obstacle representation of $\overline{K}_{7}$}
\label{fig:complement_complete}
\end{center}
\end{figure}
For complement of complete bipartite graph $\overline{K}_{n,m}$, we need at most
$O(p)$ obstacle, where $p=\max\{n,m\}$. This can be done by placing $K_n$ and
$K_m$ and separating them by a line of $O(p)$ obstacles.


\subsection{Complete binary tree}
For a complete binary tree $T$, we give an $\ell_1$-obstacle representation with $O(n\log n)$ obstacles, which is shown in Figure \ref{fig:tree}. In the figure, the Manhattan edges are shown by bold blue lines. The height and the width of the grid is $O(\log n)$ and $O(n)$ respectively. Now if we place the obstacle at every empty grid points, we get the upper bound on the $\ell_1$-obstacle number.

\begin{figure}[h]
\vspace{10pt}
\begin{center}
\includegraphics[width=7cm]{tree.pdf}
\vspace{10pt}
\caption{$\ell_1$-obstacle representation of a complete binary tree}
\label{fig:tree}
\end{center}
\end{figure}
\remove{
We can show the lower bound on the grid size to be of $\Omega(n\log n)$. The
proof is based on induction on the height of the tree. It uses the fact that all
the vertices of the bottom level can not be used to block the edges of the above
tree, because otherwise there will be a cycle. Since the height of the complete
binary tree is $\Omega(\log n)$, we get a lower bound of $\Omega(n\log n)$ which
is tight.
}


==> obstacle-high.tex <==


\section{Graphs with high $\ell_1$-obstacle number}
\label{sec:highobstacle}


In this section, we show the existence of graphs with arbitrarily large $\ell_1$-obstacle number using extremal graph theoretic tools as in \cite{PachS11}.

%\begin{wrapfigure}{r}{0.30\textwidth}
%	\vspace{-35pt}
\begin{figure}
	\begin{center}
		\includegraphics[width=3cm]{component.pdf}
		\caption{Component obstacle number of the graph is $2$.}
		\label{fig:component}
	\end{center}
\end{figure}
%	\vspace{-25pt}
%\end{wrapfigure}

We start by defining another type of obstacle, namely \emph{component obstacle number}. Let us consider an $\ell_1$-obstacle representation of a graph $G$. The representation consists of the set of vertices of $G$, a set of obstacles and also the set of Manhattan edges representing the edges of $G$. Note that, the obstacles are basically point obstacles here. We can form a single obstacle, namely \emph{component obstacle} by combining all the point obstacles that are connected through grid edges. Thus a \emph{component obstacle} is a maximally connected set of point obstacles in the unit distance graph on $\Z^2$.
The \emph{component obstacle number} is the minimum number of component obstacles needed in any $\ell_1$-obstacle representation of $G$ and it is denoted by $\ell_1$-$obs_{comp}(G)$. Figure \ref{fig:component} shows an $\ell_1$-obstacle representation of $K_4 \setminus \{e\}$, where $e=(v_1 v_4)$ along with two component obstacles that are shown in red.

%\begin{figure}[h]
%%\vspace{-35pt}
%\begin{center}
%\includegraphics[width=6.0cm]{component.pdf}
%\caption{Component obstacle number of the graph is $2$}
%\label{fig:component}
%\end{center}
%%\vspace{-20pt}
%\end{figure}


Clearly, in any $\ell_1$-obstacle representation of $G$, the number of obstacles is greater than or equal to the number of component obstacles, since each component obstacle must contain at least one obstacle. Also, the set of Manhattan edges define, in a natural sense, a set of \emph{faces} in the $\ell_1$-obstacle representation of $G$. Note that, in an $\ell_1$-obstacle representation of $G$,
\begin{enumerate}
\item each component obstacle must lie entirely in one face and
\item each non-edge of $G$ must be blocked by at least one component obstacle.
\end{enumerate}

\begin{lem}\label{lemma:obsandcompobs}
For a graph $G$ that admits an $\ell_1$-obstacle representation, if $\ell_2$-$obs(G)>1$, then $\ell_1$-$obs_{comp}(G)>1$.
\end{lem}
\begin{proof}
Let us assume that there exists a graph $G$ that admits $\ell_1$-obstacle representation and has the property that $\ell_2$-$obs(G)>1$ but $\ell_1$-$obs_{comp}(G)\leq 1$. This means at most one component obstacle is sufficient to block all the Manhattan paths between the non-adjacent vertices. If we retain the positions of the vertices and place a polygonal obstacle that contains all point obstacles, then that obstacle can block all $\ell_2$ paths between non-adjacent vertices. This happens because each $\ell_2$ path between $u$ and $v$ is totally contained inside the region defined by the set of all $\ell_1$ paths between $u$ and $v$. Hence $\ell_2$-$obs(G)\leq 1$ which is a contradiction.
\end{proof}
Using the concept of component obstacles, next we show the existence of graphs with arbitrarily large $\ell_1$-obstacle number. First we state some results in extremal graph theory.

Let $\mathscr{P}$ be a non-trivial hereditary graph property and $\mathscr{G}_{\mathscr{P}}^n$ denote the set of all graphs on $n$ labeled vertices that satisfies the property $\mathscr{P}$. Also assume that $\mathscr{G_P} = \bigcup\limits_{n\geq 1} \mathscr{G}_{\mathscr{P}}^n$. A graph is \emph{$(r,s)$-colorable}~\cite{BollobasThomason:1997} if the vertices can be partitioned into $s$ number of cliques and $(r-s)$ number of independent sets. Let $\mathscr{G}_n(r,s)$ be the set of all $(r, s)$-colorable graphs with $n$ vertices, i.e.,
$$ \mathscr{G}_n(r,s) = \{H | \mbox{$H$ has $n$ vertices and $H$ is $(r,s)$-colorable}\}$$
Hence, the set of all $(r,s)$-colorable graphs is $ \mathscr{G}(r,s) = \bigcup\limits_{n\geq 1} \mathscr{G}_n(r,s) $.
The \emph{coloring number} \cite{BollobasThomason:1997} $r(\mathscr{P})$ of a non-trivial hereditary graph property $\mathscr{P}$ is defined as
$$r(\mathscr{P})= \max\{r| \mbox{there exists some $s$ such that $\mathscr{G}(r,s) \subseteq \mathscr{G_P}$ } \}. $$
Note that, since $\mathscr{P}$ is non-trivial, $r(\mathscr{P})$ is finite. Also, since the only $(1,0)$-colorable graphs are empty and the only $(1,1)$-colorable graphs are complete graphs, $r(\mathscr{P})\geq 1$. The following theorem bounds the size of $\mathscr{G}_{\mathscr{P}}^n$.
\begin{theo}\label{theo: r,p-colorable} \cite{BollobasThomason:1997}
For any non-trivial hereditary graph property $\mathscr{P}$, we have
$|\mathscr{G}_{\mathscr{P}}^n| = 2^{(1- \frac{1}{r(\mathscr{P})}+ o(1)) \binom{n}{2}}$.
\end{theo}

Next we bound the number of graphs on $n$ vertices with component obstacle number at most $h$, for any integer $h$.

\begin{lem}
For any fixed positive integer $h$, the number of graphs on $n$ (labeled) vertices with component obstacle number at most $h$ is at most $2^{o(n^2)}$.
\end{lem}
\begin{proof}
Let us consider the property $\mathscr{P}$ to be that the graph $G$ admits a component obstacle representation with at most $1$ component obstacle. Clearly, $\mathscr{P}$ is a hereditary property. We know that there exists a bipartite graph, a split graph and a complement of a bipartite graph with $\ell_2$-obstacle number greater than $1$~\cite{AlpertKL10,MukkamalaPS-largeobs-10}, i.e., there exist $(2,0)$, $(2,1)$ and $(2,2)$-colorable graphs whose $\ell_2$-obstacle number is greater than $1$. Now by Lemma \ref{lemma:obsandcompobs}, for those graphs, component obstacle number is also greater than $1$. Note that if for some $r$ there is no $s$ such that $\mathscr{G}(r,s) \subseteq \mathscr{G_P}$, then for every $r'>r$ there is no $s'$ such that $\mathscr{G}(r',s') \subseteq \mathscr{G_P}$. Therefore, the coloring number of $\mathscr{P}$, $r(\mathscr{P})$ is $1$. By Theorem \ref{theo: r,p-colorable}, we have $|\mathscr{G_P}^n|= 2^{o(n^2)}$. Therefore, for $h=1$, the number of graphs on $n$ labeled vertices with component obstacle number at most $1$ is $2^{o(n^2)}$.

Let us consider that $G$ is a graph on $n$ labeled vertices that admits a component obstacle representation with $h$ component obstacles. Let $O_1, O_2, \ldots, O_h$ be the component obstacles of $G$. For each $1\leq i\leq h$, consider $G_i$ to be the visibility graphs on $n$ labeled vertices with component obstacle $O_i$. The vertex position of $G_i$ is the same as the vertex positions of $G$. Clearly, edge set of $G$, $E(G)= \bigcap\limits_{i=1}^{h} E(G_i)$, where $E(G_i)$ is the edge set of $G_i$. Note that each $G_i$ has component obstacle number at most $1$ and by previous argument, we have, number of such graphs on $n$ labeled vertices is $2^{o(n^2)}$. Hence, the number of graphs on $n$ labeled vertices having component obstacle number at most $h$ is at most $2^{ho(n^2)}=2^{o(n^2)}$.
\end{proof}


Since number of graphs (or bipartite graphs) with $n$ labeled vertices is $2^{\binom{n}{2}}$ (or $\Omega(2^{(n^2/4)})$ respectively), we have the following theorem.

\begin{theo}
For any fixed positive integer $h$, there exist graphs (bipartite graphs) with component obstacle number at least $h$.
\end{theo}

Moreover, since for any graph $G$, $\ell_1$-$obs(G)\geq \ell_1$-$obs_{comp}(G)$, we have the following corollary of the above theorem.

\begin{coro}
For any fixed positive integer $h$, there exist graphs (bipartite graphs) with
$\ell_1$-obstacle number at least $h$.
\end{coro}



==> obstacle-impossible.tex <==

%\section{Impossibility results}
%\label{sec:impossible}
%In this section, we focus on the embeddability problem of graphs in $\mathbb{Z}^2$. We show that, in certain cases, we can not have an $\ell_1$-obstacle representation.
%\subsection{Finite grid}
%Here we show that every graph can not be embedded in a finite grid.
%
%\begin{theo}\label{theo:impossiblegraph}
%There exists a $n_0 \in \mathbb{N}$ such that for all $ n > n_0$, there exists a graph with $n$ vertices that can not be embedded in an $l \times b$ grid where $lb=N=o(n^2)$.
%\end{theo}
%\begin{proof}
% The number of labeled graphs that admits $\ell_1$ representation in an $l \times b$ grid is at most $\binom{N}{n}n!2^{N-n}(\leq n! 2^{2N-n})$ because we can select $n$ positions for the vertices of the graph in $\binom {N} {n}$ ways and vertex positions can be permuted in $n!$ ways and then we can place the obstacles in remaining $N-n$ grid points in $2^{N-n}$ ways. On the other hand, the number of non-isomorphic graphs possible with $n$ vertices is at least $\frac{2^{\binom {n}{2}}}{n!}$ \cite{Matousek:1998}. If all graphs with $n$ vertices are embeddable in the  grid of size $N$, then for  all $n > n_{0}$, we have
%$2^{2N-n}n! \geq {2^{\binom {n}{2}}}/{n!}
%\Rightarrow N = \Omega(n^2)$,
%where $n_0$ is a function of constants involved in   $\binom{n}{2} =\Omega(n^2)$ and $\log (n!)= O(n \log n).$
%\qed \end{proof}
%
%Next theorem shows that if the obstacle number is bounded, then to have an $\ell_1$-obstacle representation, we need a large grid.
%
%
%\begin{theo}\label{theo:impossiblegraphwithobstacle}
% If all graphs with $n$ vertices can be embedded in a grid of size $N$ using $h$ obstacles, then $ N \gtrsim ({\frac{2^{n^2}}{(n!)^2}})^{\frac{1}{n+h}}(n+h)$.
%\end{theo}
%\begin{proof}
%The number of labeled graphs that can be embedded in a grid of size $N$ using $h$ obstacles is at most $\binom{N}{n+h}n!$ and the number of non-isomorphic graphs possible with $n$ vertices is at least $\frac{2^{\binom {n}{2}}}{n!}$~\cite{Matousek:1998}. Hence,
%$$\binom{N}{n+h}n! \geq \frac{2^{\binom {n}{2}}}{n!} \Rightarrow (\frac{Ne}{n+h})^{n+h} \geq \frac{2^{\binom {n}{2}}}{(n!)^2} \Rightarrow N \gtrsim ({\frac{2^{n^2}} {(n!)^2}})^{\frac{1}{n+h}}(n+h). ~~~~~~\qed $$
%
%\end{proof}
%
%For $h=O(n)$ and $h=O(n\log n)$, we have the following,
%
%\begin{coro}
%\begin{enumerate}
%	\item[(i)]	
%	 There exists a graph with $n$ vertices that can not be embedded using $O(n)$ obstacles in an $l \times b$ grid where $lb=N=2^{o(n)}$.
%	
%	 \item[(ii)]
%There exists a graph with $n$ vertices that can not be embedded using $O(n \log n)$ obstacles in an $l \times b$ grid where $lb=N=2^{o(\frac{n}{\log n})}$.
%	
%\end{enumerate}
%\end{coro}

\section{Strip representation}
\label{sec:horizontal_grid}

%\begin{figure}[h]
%%\vspace{-25pt}
%\begin{center}
%\includegraphics[width=7cm]{envelop.pdf}
%\caption{Maintaining the upper and lower envelops of ${\cP}_{i,j}$ in $T$.}
%\label{fig:envelop}
%\end{center}
%%\vspace{-30pt}
%\end{figure}



\begin{wrapfigure}{r}{0.50\textwidth}
	\vspace{-15pt}
	\begin{center}
		\includegraphics[width=6.0cm]{envelop.pdf}
		\caption{Maintaining the upper and lower envelopes of ${\cP}_{i,j}$ in $T$.}
		\label{fig:envelop}
	\end{center}
	\vspace{-5pt}
\end{wrapfigure}



In this section, we study the $\ell_1$-obstacle representation of a graph $G$ in a \emph{horizontal strip}. A \emph{horizontal strip} is a grid where the $y$-coordinates are bounded but the $x$-coordinates can be any arbitrary integer. We present a compression technique to show that every graph does not admit an $\ell_1$-obstacle representation in this case. The case of \emph{vertical strip} can be argued in a similar way. Note that an $\ell_1$-obstacle representation in a horizontal strip for a graph implies its $\ell_1$-obstacle representation in $\Z^2$. But the converse is not true. For example, $C_n$ and $K_n$, for $n>4$, admit $\ell_1$-obstacle representation in $\Z^2$ (see Appendix~\ref{app:examplesgridrepresentation}) but not $\ell_1$-obstacle representations in horizontal strips containing only two rows.

First we show that if a graph admits an $\ell_1$-obstacle representation in a horizontal strip, it admits an $\ell_1$-obstacle representation in a finite grid.

\begin{lem}\label{lemma:finitehorizontalembed}
Let $G$ admit an $\ell_1$-obstacle representation in a horizontal strip of height $b$. Then $G$ can have an $\ell_1$-obstacle representation in a finite grid of size $b \times O(b^3n)$.
\end{lem}



\begin{proof}
%\noindent {\em Proof.}
Let $embd(G)$ be the $\ell_1$-obstacle representation of $G$ in a horizontal strip of height $b$. For ease of exposition, we prove the theorem for the case where every vertex of $G$ has different $x$-coordinates in $embd(G)$. The same argument holds for the case where some vertices have same $x$-coordinates. We say two vertices $v_1$ and $v_2$ are consecutive if there is no other vertex whose $x$-coordinate lies between the $x$-coordinates of $v_1$ and $v_2$. If for any two consecutive vertices in $embd(G)$, the difference between their $x$-coordinates is less than $O(b^3)$, then the theorem is immediate. Hence, we aim to prove, by a compression argument, that there exists an $\ell_1$-obstacle representation of $G$ in a horizontal strip of height $b$ such that
\begin{itemize}
\item the consecutive vertices of $G$ in $embd(G)$ remain consecutive in the new representation, and
\item the difference between $x$-coordinates of two consecutive vertices is $O(b^3)$.
\end{itemize}



For the rest of the proof, we focus on the portion, say $T$ of $embd(G)$ between two consecutive vertices of $G$. We modify each of these portions to get a different representation of $G$ in the same horizontal strip. The modification is as follows.
Let $l$ and $r$ be the starting and ending vertical lines of $T$, respectively. Note that both $l$ and $r$ have $b$ grid points each. In $embd(G)$, there may be multiple Manhattan paths from a grid point of $l$ to a grid point of $r$. Let ${\cP}(i,j)$ denote the set of all Manhattan paths from $i$-th grid point of $l$ to
$j$-th grid point of $r$. In the new representation, we only maintain the upper and lower envelope of each ${\cP}(i,j)$ and color those paths as shown in Figure \ref{fig:envelop}. In $T$, we retain all the colored paths and put obstacles everywhere else. Let us denote this new representation by $embd'(G)$. Note that, in $embd'(G)$, the connectivity between $i$-th grid point of $l$ and $j$-th
grid point of $r$ is maintained, if $P(i,j)$ is non-empty. Also, putting obstacles does not create any unwanted connectivity. Hence, we have the following claim:


%\begin{wrapfigure}{l}{0.40\textwidth}
%\vspace{-25pt}
%\begin{center}
%\includegraphics[width=3.5cm]{envelop.pdf}
%\caption{Maintaining the upper and lower envelops of $P_{i,j}$}
%\label{fig:envelop}
%\end{center}
%\vspace{-30pt}
%\end{wrapfigure}



\begin{cl}
The new representation $embd'(G)$ is an $\ell_1$-obstacle representation of $G$.
\end{cl}

Next we calculate the total number of \emph{bend points} of $embd'(G)$.
A \emph{bend point} of $embd'(G)$ is a grid point on some colored path $\cP$
where $\cP$ changes direction. Since the height of the grid is bounded by $b$, the number of bend points on a colored path is at most $2b-2$. Moreover, every bend point is on some colored path that defines either an upper or a lower envelope of some $\cP(i,j)$. Since there are at most $O(b^2)$ non-empty $\cP(i,j)$s, the total number of bend points is $O(b^3)$ in $T$.

Two bend points $b_1$ and $b_2$ are consecutive if there is no other bend point whose $x$-coordinate lies between the $x$-coordinates of $b_1$ and $b_2$. The following claim, proved later, shows that the horizontal distance between two consecutive bend points need not be arbitrarily large.
\begin{cl}
The representation $embd'(G)$ can be modified to another representation $embd''(G)$ where the number of vertical lines between two consecutive bend points is constant.
\label{cl:embed2}
\end{cl}
So, in the representation $embd''(G)$, the total number of bend points is $O(b^3)$ and between two consecutive bend points, we have only one vertical grid line. Hence, there are $O(b^3)$ vertical grid lines between any two consecutive vertices. Therefore, $embd''(G)$ is of the size $b \times O(b^3n)$.
\end{proof}

\begin{figure}[h]
%\vspace{-25pt}
\begin{center}
\includegraphics[width=6.5cm]{compression.pdf}
\caption{Illustration of compression}
\label{fig:compression}
\end{center}
%\vspace{-30pt}
\end{figure}

\begin{proof}[Proof of Claim~\ref{cl:embed2}]
In $embd'(G)$, note that, all the colored paths that cross the section between two consecutive bend points, are horizontal. \remove{That is, all the paths start at some $y$-coordinate of the left vertical grid line of the section and end at the same $y$-coordinate of the right vertical grid line of the section.} The vertical grid lines between two consecutive bend points can be compressed to only three vertical grid lines such that the first and the third vertical grid line is identical with the first and last vertical grid line of the section. In the middle grid line, we put obstacles at those $y$-coordinates through which there is no path that passes through the same $y$-coordinate in the first vertical grid line as shown in Figure \ref{fig:compression}. Repeating this process for every consecutive bend points, we have an $embd''(G)$ where the number of vertical lines between two consecutive bend points is constant.
\end{proof}
%From Theorem \ref{theo:impossiblegraph} and Lemma \ref{lemma:finitehorizontalembed}, we have the following corollary
%\begin{coro}
%There exists graphs that can not have an $\ell_1$-obstacle representation in horizontal grid of height $o(n^{1/4})$.
%\end{coro}



==> obstacle-observe.tex <==

\section{Observations and open problems}
\label{app:open}
Here, we highlight some important observations and propose some interesting problems. In this article, we have shown that some graphs (e.g. planar) admit grid obstacle representation in $\mathbb{Z}^2$. On the negative side, it has been shown that there exist graphs that do not admit grid obstacle representation in $\mathbb{Z}^2$. Hence, perhaps the most interesting question to ask is the following.

\begin{prob}
Characterize the graphs that admit grid obstacle representation in $\mathbb{Z}^2$.
\end{prob}

There are mainly two optimality problems associated with $\ell_1$-obstacle representation of a graph. The problems are as follows:

\begin{prob}
Given a graph $G$ that admits $\ell_1$-obstacle representation, find the $\ell_1$-obstacle number of $G$ on $\mathbb{Z}^2$.
\end{prob}

\begin{prob}
Given a graph $G$ that admits $\ell_1$-obstacle representation, find the minimum grid size for $\ell_1$-obstacle representation of $G$ on $\mathbb{Z}^2$.
\end{prob}

By simple counting techniques, it can be shown that if we have a bound on
the $\ell_1$-obstacle number, then there exist some graphs that can not be
embedded in a small grid. This indicates a dual nature between the above two
problems. Hence, the following bicriterion problem is interesting to study.


\begin{prob}
Given a graph $G$ that admits $\ell_1$-obstacle representation, find the representation of $G$ on $\mathbb{Z}^2$ that minimizes both the grid size as well as the $\ell_1$-obstacle number.
\end{prob}

%\subsection{Problems related to $\ell_1$-obstacle representation}
%\label{ssec:open:existence}
%By Theorem \ref{theo:InZ3}, we have seen that every graph admits
%$\ell_1$-obstacle representation on $\mathbb{Z}^3$. We have also shown the
%$\ell_1$-obstacle representation of planar and outerplanar graphs on
%$\mathbb{Z}^2$. Perhaps the most important question to ask is the following.
%
%\begin{prob}
%%\paragraph{\bf Problem 1:}
%Does every graph (bipartite) admit $\ell_1$-obstacle representation in $\mathbb{Z}^2$?
%\end{prob}
%
%%We also propose the following problem for bipartite graph.
%%
%%{\bf Problem 2:} Does every bipartite graph admit $\ell_1$-obstacle representation in $\mathbb{Z}^2$?
%\remove{
%If Problem 2 is answered positively, then we have positive answer for Problem 1
%using the construction based on \complain{\emph{Horton set} \citep{}}.}
%
%
%By Theorem \ref{theo:impossiblegraph} and
%\ref{theo:impossiblegraphwithobstacle}, we feel that there exists graphs that do
%not admit $\ell_1$-obstacle representation in $\mathbb{Z}^2$.
%Next, we pose a rather simple question where the mapping of vertices to grids
%is given.
%
%\begin{prob}
%%\paragraph{\bf Problem 2:}
%Given a graph $G=(V,E)$ and an injective mapping $f: V \rightarrow \mathbb{Z}^2$, does there exist an $\ell_1$-obstacle representation on $\mathbb{Z}^2$?
%\end{prob}
%
%
%It is easy to observe that not every graph admits an $\ell_1$-obstacle representation if the vertex mapping is given. For example, if the vertices are mapped to consecutive grid points of a horizontal of vertical line, then the only representable graph is $P_n$, path with $n$ vertices. To this end, we obtain a forbidden structure $\mathcal{F}$ depending on both the vertex mapping and the edge set of $G$. Let us assume that four vertices of $G$, say $v_i, v_j, v_k$ and $v_l$ are mapped to the grid in such a way that $R(v_i,v_j)\setminus R(v_k,v_l)$ and $R(v_k,v_l)\setminus R(v_i,v_j)$ both are disconnected, where $R(v_i,v_j)$ is the rectangle with $v_i$ and $v_j$ being its two opposite corner vertices (see Figure \ref{fig:forbiddenstructure}).
%
%\begin{figure}[!h]
%\begin{center}
%\includegraphics[width=4cm]{forbid.pdf}
%\caption{Forbidden structure for Problem 3}
%\label{fig:forbiddenstructure}
%\end{center}
%\end{figure}
%
%Now if $(1)$ $v_iv_j, v_kv_l \in E$ and $(2)$ $v_iv_l \notin E$ or $v_kv_j \notin E$, then the graph $G$ does not have an $\ell_1$-obstacle representation. Because, the Manhattan paths $P_{ij}$ between $v_i$ and $v_j$, and $P_{kl}$ between $v_k$ and $v_l$ must intersect at some grid point. This creates Manhattan paths between $v_i$ and $v_l$ and also between $v_k$ and $v_j$. This forbidden structure $\mathcal{F}$ is illustrated in  \ref{fig:forbiddenstructure}. But this may not be the only forbidden structure for $\ell_1$-obstacle representation of $G$ with a given vertex mapping. Hence, we pose the following problem.
%
%\begin{prob} Given a vertex mapping of $G$ into $\mathbb{Z}^2$, find all the
%forbidden structures for the existence of $\ell_1$-obstacle representation of
%$G$.
%\end{prob}



%\subsection{Effect of graph operations on $\ell_1$-obstacle representation}
%\label{ssec:open:operations}
%
%To understand the nature of the embeddabilty problem, we need to focus on the
%following fundamental problem.
%
%\begin{prob}
%If $G$ admits an $\ell_1$-obstacle representation on $\mathbb{Z}^2$, then does $G'=G \cup \{e\}$ admit an $\ell_1$-obstacle representation?
%\end{prob}
%
%
%If this problem is answered positively, then we can show the existence of
%$\ell_1$-obstacle representation of any graph $G$ by repeatedly adding edges to
%some planar graph, which is embeddable by Corollary \ref{coro:planar}.
%Similarly, we can show the existence of $\ell_1$-obstacle representation of any
%graph $G$ by repeatedly deleting edges from a complete graph, if the following
%problem is answered positively.
%
%\begin{prob} If $G$ admits an $\ell_1$-obstacle representation on $\mathbb{Z}^2$, then does $G'=G \setminus \{e\}$ admit an $\ell_1$-obstacle representation?
%\end{prob}
%
%If there exists some graphs that do not admit $\ell_1$-obstacle representation, then we might construct an infinite family of graphs that do not admit $\ell_1$-obstacle representation by studying the behavior under different graph operations. Hence, it is worth studying the following problem.
%
%\begin{prob}
%Does the existence of $\ell_1$-obstacle representation change under different graph products like Cartesian product, tensor product or strong product?
%\end{prob}
%




%\subsection{Complexity of optimum $\ell_1$-obstacle representation}
%\label{ssec:open:complexity}
%There are mainly two optimality problems associated with $\ell_1$-obstacle representation of a graph. The problems are as follows:
%
%\begin{prob}
%Given a graph $G$ that admits $\ell_1$-obstacle representation, find the $\ell_1$-obstacle number of $G$ on $\mathbb{Z}^2$.
%\end{prob}
%
%\begin{prob}
%Given a graph $G$ that admits $\ell_1$-obstacle representation, find the minimum grid size for $\ell_1$-obstacle representation of $G$ on $\mathbb{Z}^2$.
%\end{prob}
%
%Theorem \ref{theo:impossiblegraphwithobstacle} says that if we have a bound on
%the $\ell_1$-obstacle number, then there exist some graphs that can not be
%embedded in a small grid. This indicates a dual nature between the above two
%problems. Hence, the following bicriterion problem is interesting to study.
%
%
%\begin{prob}
%Given a graph $G$ that admits $\ell_1$-obstacle representation, find the representation of $G$ on $\mathbb{Z}^2$ that minimizes both the grid size as well as the $\ell_1$-obstacle number.
%\end{prob}


==> obstacle-strip.tex <==

%\section{Impossibility results}
%\label{sec:impossible}
%In this section, we focus on the embeddability problem of graphs in $\mathbb{Z}^2$. We show that, in certain cases, we can not have an $\ell_1$-obstacle representation.
%\subsection{Finite grid}
%Here we show that every graph can not be embedded in a finite grid.
%
%\begin{theo}\label{theo:impossiblegraph}
%There exists a $n_0 \in \mathbb{N}$ such that for all $ n > n_0$, there exists a graph with $n$ vertices that can not be embedded in an $l \times b$ grid where $lb=N=o(n^2)$.
%\end{theo}
%\begin{proof}
% The number of labeled graphs that admits $\ell_1$ representation in an $l \times b$ grid is at most $\binom{N}{n}n!2^{N-n}(\leq n! 2^{2N-n})$ because we can select $n$ positions for the vertices of the graph in $\binom {N} {n}$ ways and vertex positions can be permuted in $n!$ ways and then we can place the obstacles in remaining $N-n$ grid points in $2^{N-n}$ ways. On the other hand, the number of non-isomorphic graphs possible with $n$ vertices is at least $\frac{2^{\binom {n}{2}}}{n!}$ \cite{Matousek:1998}. If all graphs with $n$ vertices are embeddable in the  grid of size $N$, then for  all $n > n_{0}$, we have
%$2^{2N-n}n! \geq {2^{\binom {n}{2}}}/{n!}
%\Rightarrow N = \Omega(n^2)$,
%where $n_0$ is a function of constants involved in   $\binom{n}{2} =\Omega(n^2)$ and $\log (n!)= O(n \log n).$
%\qed \end{proof}
%
%Next theorem shows that if the obstacle number is bounded, then to have an $\ell_1$-obstacle representation, we need a large grid.
%
%
%\begin{theo}\label{theo:impossiblegraphwithobstacle}
% If all graphs with $n$ vertices can be embedded in a grid of size $N$ using $h$ obstacles, then $ N \gtrsim ({\frac{2^{n^2}}{(n!)^2}})^{\frac{1}{n+h}}(n+h)$.
%\end{theo}
%\begin{proof}
%The number of labeled graphs that can be embedded in a grid of size $N$ using $h$ obstacles is at most $\binom{N}{n+h}n!$ and the number of non-isomorphic graphs possible with $n$ vertices is at least $\frac{2^{\binom {n}{2}}}{n!}$~\cite{Matousek:1998}. Hence,
%$$\binom{N}{n+h}n! \geq \frac{2^{\binom {n}{2}}}{n!} \Rightarrow (\frac{Ne}{n+h})^{n+h} \geq \frac{2^{\binom {n}{2}}}{(n!)^2} \Rightarrow N \gtrsim ({\frac{2^{n^2}} {(n!)^2}})^{\frac{1}{n+h}}(n+h). ~~~~~~\qed $$
%
%\end{proof}
%
%For $h=O(n)$ and $h=O(n\log n)$, we have the following,
%
%\begin{coro}
%\begin{enumerate}
%	\item[(i)]	
%	 There exists a graph with $n$ vertices that can not be embedded using $O(n)$ obstacles in an $l \times b$ grid where $lb=N=2^{o(n)}$.
%	
%	 \item[(ii)]
%There exists a graph with $n$ vertices that can not be embedded using $O(n \log n)$ obstacles in an $l \times b$ grid where $lb=N=2^{o(\frac{n}{\log n})}$.
%	
%\end{enumerate}
%\end{coro}

\section{Strip representation}
\label{sec:horizontal_grid}

%\begin{figure}[h]
%%\vspace{-25pt}
%\begin{center}
%\includegraphics[width=7cm]{envelop.pdf}
%\caption{Maintaining the upper and lower envelops of ${\cP}_{i,j}$ in $T$.}
%\label{fig:envelop}
%\end{center}
%%\vspace{-30pt}
%\end{figure}







In this section, we study the $\ell_1$-obstacle representation of a graph $G$ in a \emph{horizontal strip}. A \emph{horizontal strip} is a grid where the $y$-coordinates are bounded but the $x$-coordinates can be any arbitrary integer. We present a compression technique to show that every graph does not admit an $\ell_1$-obstacle representation in this case. The case of \emph{vertical strip} can be argued in a similar way. Note that an $\ell_1$-obstacle representation in a horizontal strip for a graph implies its $\ell_1$-obstacle representation in $\Z^2$. But the converse is not true. For example, $C_n$ and $K_n$, for $n>4$, admit $\ell_1$-obstacle representation in $\Z^2$ but not $\ell_1$-obstacle representations in horizontal strips containing only two rows.

\begin{wrapfigure}{r}{0.50\textwidth}
	\vspace{-5pt}
	\begin{center}
		\includegraphics[width=5.0cm]{envelop.pdf}
		\caption{Maintaining the upper and lower envelopes of ${\cP}_{i,j}$ in $T$.}
		\label{fig:envelop}
	\end{center}
	\vspace{-10pt}
\end{wrapfigure}
First we show that if a graph admits an $\ell_1$-obstacle representation in a horizontal strip, it admits an $\ell_1$-obstacle representation in a finite grid.

\begin{theo}\label{lemma:finitehorizontalembed}
Let $G$ admit an $\ell_1$-obstacle representation in a horizontal strip of height $b$. Then $G$ can have an $\ell_1$-obstacle representation in a finite grid of size $b \times O(b^3n)$.
\end{theo}



\begin{proof}
%\noindent {\em Proof.}
Let $embd(G)$ be the $\ell_1$-obstacle representation of $G$ in a horizontal strip of height $b$. For ease of exposition, we prove the theorem for the case where every vertex of $G$ has different $x$-coordinates in $embd(G)$. The same argument holds for the case where some vertices have same $x$-coordinates. We say two vertices $v_1$ and $v_2$ are consecutive if there is no other vertex whose $x$-coordinate lies between the $x$-coordinates of $v_1$ and $v_2$. If for any two consecutive vertices in $embd(G)$, the difference between their $x$-coordinates is less than $O(b^3)$, then the theorem is immediate. Hence, we aim to prove, by a compression argument, that there exists an $\ell_1$-obstacle representation of $G$ in a horizontal strip of height $b$ such that
\begin{itemize}
\item the consecutive vertices of $G$ in $embd(G)$ remain consecutive in the new representation, and
\item the difference between $x$-coordinates of two consecutive vertices is $O(b^3)$.
\end{itemize}



For the rest of the proof, we focus on the portion, say $T$ of $embd(G)$ between two consecutive vertices of $G$. We modify each of these portions to get a different representation of $G$ in the same horizontal strip. The modification is as follows.
Let $l$ and $r$ be the starting and ending vertical lines of $T$, respectively. Note that both $l$ and $r$ have $b$ grid points each. In $embd(G)$, there may be multiple Manhattan paths from a grid point of $l$ to a grid point of $r$. Let ${\cP}(i,j)$ denote the set of all Manhattan paths from $i$-th grid point of $l$ to
$j$-th grid point of $r$. In the new representation, we only maintain the upper and lower envelope of each ${\cP}(i,j)$ and color those paths as shown in Figure \ref{fig:envelop}. In $T$, we retain all the colored paths and put obstacles everywhere else. Let us denote this new representation by $embd'(G)$. Note that, in $embd'(G)$, the connectivity between $i$-th grid point of $l$ and $j$-th
grid point of $r$ is maintained, if $P(i,j)$ is non-empty. Also, putting obstacles does not create any unwanted connectivity. Hence, we have the following claim:


%\begin{wrapfigure}{l}{0.40\textwidth}
%\vspace{-25pt}
%\begin{center}
%\includegraphics[width=3.5cm]{envelop.pdf}
%\caption{Maintaining the upper and lower envelops of $P_{i,j}$}
%\label{fig:envelop}
%\end{center}
%\vspace{-30pt}
%\end{wrapfigure}



\begin{cl}
The new representation $embd'(G)$ is an $\ell_1$-obstacle representation of $G$.
\end{cl}

Next we calculate the total number of \emph{bend points} of $embd'(G)$.
A \emph{bend point} of $embd'(G)$ is a grid point on some colored path $\cP$
where $\cP$ changes direction. Since the height of the grid is bounded by $b$, the number of bend points on a colored path is at most $2b-2$. Moreover, every bend point is on some colored path that defines either an upper or a lower envelope of some $\cP(i,j)$. Since there are at most $O(b^2)$ non-empty $\cP(i,j)$s, the total number of bend points is $O(b^3)$ in $T$.

Two bend points $b_1$ and $b_2$ are consecutive if there is no other bend point whose $x$-coordinate lies between the $x$-coordinates of $b_1$ and $b_2$. The following claim, proved later, shows that the horizontal distance between two consecutive bend points need not be arbitrarily large.
\begin{figure}[h]
%\vspace{-25pt}
\begin{center}
\includegraphics[width=8cm]{compression.pdf}
\caption{Illustration of compression}
\label{fig:compression}
\end{center}
%\vspace{-30pt}
\end{figure}

\begin{cl}
The representation $embd'(G)$ can be modified to another representation $embd''(G)$ where the number of vertical lines between two consecutive bend points is constant.
\label{cl:embed2}
\end{cl}
So, in the representation $embd''(G)$, the total number of bend points is $O(b^3)$ and between two consecutive bend points, we have only one vertical grid line. Hence, there are $O(b^3)$ vertical grid lines between any two consecutive vertices. Therefore, $embd''(G)$ is of the size $b \times O(b^3n)$.
\end{proof}


\begin{proof}[Proof of Claim~\ref{cl:embed2}]
In $embd'(G)$, note that, all the colored paths that cross the section between two consecutive bend points, are horizontal. \remove{That is, all the paths start at some $y$-coordinate of the left vertical grid line of the section and end at the same $y$-coordinate of the right vertical grid line of the section.} The vertical grid lines between two consecutive bend points can be compressed to only three vertical grid lines such that the first and the third vertical grid line is identical with the first and last vertical grid line of the section. In the middle grid line, we put obstacles at those $y$-coordinates through which there is no path that passes through the same $y$-coordinate in the first vertical grid line as shown in Figure \ref{fig:compression}. Repeating this process for every consecutive bend points, we have an $embd''(G)$ where the number of vertical lines between two consecutive bend points is constant. 
\end{proof}


%From Theorem \ref{theo:impossiblegraph} and Lemma \ref{lemma:finitehorizontalembed}, we have the following corollary
\remove{
\begin{theo}
There exists graphs that can not have an $\ell_1$-obstacle representation in horizontal grid of height $o(n^{1/4})$.
\end{theo}
\begin{proof}
First we show that there exists a $n_0 \in \mathbb{N}$ such that for all $ n > n_0$, there exists a graph with $n$ vertices that can not be embedded in an $l \times b$ grid where $lb=N=o(n^2)$. The number of labeled graphs that admits $\ell_1$ representation in an $l \times b$ grid is at most $\binom{N}{n}n!2^{N-n}(\leq n! 2^{2N-n})$ because we can select $n$ positions for the vertices of the graph in $\binom {N} {n}$ ways and vertex positions can be permuted in $n!$ ways and then we can place the obstacles in remaining $N-n$ grid points in $2^{N-n}$ ways. On the other hand, the number of non-isomorphic graphs possible with $n$ vertices is at least $\frac{2^{\binom {n}{2}}}{n!}$ \cite{Matousek:1998}. If all graphs with $n$ vertices are embeddable in the  grid of size $N$, then for  all $n > n_{0}$, we have $2^{2N-n}n! \geq {2^{\binom {n}{2}}}/{n!} \Rightarrow N = \Omega(n^2)$, where $n_0$ is a function of constants involved in $\binom{n}{2} =\Omega(n^2)$ and $\log (n!)= O(n \log n).$

From Lemma \ref{lemma:finitehorizontalembed}, it is clear that if the horizontal grid has height $o(n^{1/4})$, total number of grid point becomes $o(n^2)$. Hence we have the theorem.
\end{proof}
} 
